Product-Level Try-on: Characteristics-preserving Try-on with Realistic Clothes Shading and Wrinkles

Image-based virtual try-on systems,which fit new garments onto human portraits,are gaining research attention.An ideal pipeline should preserve the static features of clothes(like textures and logos)while also generating dynamic elements(e.g.shadows,folds)that adapt to the model's pose and environment.Previous works fail specifically in generating dynamic features,as they preserve the warped in-shop clothes trivially with predicted an alpha mask by composition.To break the dilemma of over-preserving and textures losses,we propose a novel diffusion-based Product-level virtual try-on pipeline,\ie PLTON, which can preserve the fine details of logos and embroideries while producing realistic clothes shading and wrinkles.The main insights are in three folds:1)Adaptive Dynamic Rendering:We take a pre-trained diffusion model as a generative prior and tame it with image features,training a dynamic extractor from scratch to generate dynamic tokens that preserve high-fidelity semantic information. Due to the strong generative power of the diffusion prior,we can generate realistic clothes shadows and wrinkles.2)Static Characteristics Transformation: High-frequency Map(HF-Map)is our fundamental insight for static representation.PLTON first warps in-shop clothes to the target model pose by a traditional warping network,and uses a high-pass filter to extract an HF-Map for preserving static cloth features.The HF-Map is used to generate modulation maps through our static extractor,which are injected into a fixed U-net to synthesize the final result.To enhance retention,a Two-stage Blended Denoising method is proposed to guide the diffusion process for correct spatial layout and color.PLTON is finetuned only with our collected small-size try-on dataset.Extensive quantitative and qualitative experiments on 1024 768 datasets demonstrate the superiority of our framework in mimicking real clothes dynamics.

==> sections/pre_methods.tex <==
\section{Clothes Composition}
To better address the problem, we reiterate the pros and cons of the conventional design of composition-based try-on. Traditional GAN-based pipelines employ a split-transform-merge pipeline with a final alpha composition to fuse all image components to generate a synthetic clothed person. As proposed by VITON~\cite{VITON}, alpha masks help composite deformed clothing images with rendered coarse images. Due to the randomness of logos and embroidery, it is almost impossible to generate the full features of the target clothes without a synthetic mask. This acknowledgment seems to dominate the current try-in pipeline design, severely hindering the development of the field.
As shown in figure ~\ref{fig:teaser} and figure ~\ref{fig:introduction}, it is incredibly challenging to preserve the fine details of the target clothing while generating coherent clothes shadows and wrinkles on the reference person. Our primary motivation is to break this dilemma and design a new paradigm to replace the traditional design of a product-level try-on application.
